An Extended Catalogue of galaxy morphology using Deep Learning in Southern Photometric Local Universe Survey Data Release 3

The morphological diversity of galaxies is a relevant probe of galaxy evolution and cosmological structure formation. However, in large sky surveys, even the morphological classification of galaxies into two classes, like late-type (LT) and early-type (ET), still represents a significant challenge. In this work we present a Deep Learning (DL) based morphological catalog built from images obtained by the Southern Photometric Local Universe Survey (S-PLUS) Data Release 3 (DR3). Our DL method achieves an precision rate of 98.5$\%$ in accurately distinguishing between spiral, as part of the larger category of late type (LT) galaxies, and elliptical, belonging to early type (ET) galaxies. Additionally, we have implemented a secondary classifier that evaluates the quality of each galaxy stamp, which allows to select only high-quality images when studying properties of galaxies on the basis of their DL morphology. From our LT/ET catalog of galaxies, we recover the expected color--magnitude diagram in which LT galaxies display bluer colors than ET ones. Furthermore, we also investigate the clustering of galaxies based on their morphology, along with their relationship to the surrounding environment. As a result, we deliver a full morphological catalog with $164314$ objects complete up to $r_{petro}<18$, covering $\sim 1800$ deg$^2$, including a significant area of the Southern hemisphere that was not covered by previous morphology catalogues.

==> extras.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\title[Deep Learning Analysis of Strong Lenses]{Deep Learning Analysis of Strong Lenses in Wide-field Surveys}


%\include{authors}


% These dates will be filled out by the publisher
%\date{Accepted XXX. Received YYY; in original form ZZZ}

% Enter the current year, for the copyright statements etc.
%\pubyear{2019}

% Don't change these lines
%\begin{document}
%\label{firstpage}
%\pagerange{\pageref{firstpage}--\pageref{lastpage}}
%\maketitle

% Abstract of the paper
%\begin{abstract}
%\begin{itemize}
%    \item Measuring lenses in large, wide-field surveys is expensive.
%    \item Use regression analysis in deep learning to measure four parameters of lenses simulated for ground-based surveys.
%    \item We can measure ground-based-observations of lenses with estimates of uncertainties.
%    \item These measurements are competitive with ...
%\end{itemize}
%\end{abstract}

% Select between one and six entries from the list of approved keywords.
% Don't make up new ones.
%\begin{keywords}
%gravitational lensing -- strong lensing -- machine learning
%\end{keywords}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%% BODY OF PAPER %%%%%%%%%%%%%%%%%%



%\affiliation[1]{Centro Federal de Educa\c{c}\~ao Tecnol\'ogica Celso Suckow da Fonseca, Rodovia M\'ario Covas,lote J2, quadra J, CEP 23810-000,  Itagua\'i, RJ, Brazil}
%\affiliation[2]{Centro Brasileiro de Pesquisas F\'isicas, Rua Dr. Xavier Sigaud 150, CEP 22290-180, Rio de Janeiro, RJ, Brazil}
%\affiliation[3]{Fermi National Accelerator Laboratory, Batavia, IL, U.S.A.}
%\affiliation[4]{Dipartimento di Fisica e Scienze della Terra, Universita degli Studi di Ferrara, Via Saragat 1, I-44122 Ferrara, Italy}
%\affiliation[5]{Faculty of Science and Engineering, University of Groningen, Nijenborgh 4, 9747 AG Groningen, The Netherlands}
%\affiliation[6]{Centre for Cosmology, Particle Physics and Phenomenology, Institute of Mathematics and Physics, Louvain University, 2 Chemin du Cyclotron, 1348 Louvain-la-Neuve, Belgium}
%\affiliation[7]{Institut d'Astrophysique de Paris, GReCO, UMR7095 CNRS, 98 bis boulevard Arago, 75014 Paris, France}
%\affiliation[8]{Laboratoire d'Annecy de Physique des Particules (LAPP), Universit\'e Savoie Mont Blanc, CNRS/IN2P3, F-74941 Annecy, France}
%\affiliation[9]{Universidade de Bras\'ilia, Instituto de F\'isica, Caixa Postal 04455, Brasília, DF, 70919-970, Brazil}
%% End authors and affiliations in JCAP style

%\author[K. T. Smith et al.]{
%Keith T. Smith,$^{1}$\thanks{E-mail: mn@ras.org.uk (KTS)}
%A. N. Other,$^{2}$
%Third Author$^{2,3}$
%and Fourth Author$^{3}$
%\\
% List of institutions
%$^{1}$Royal Astronomical Society, Burlington House, Piccadilly, London W1J 0BQ, UK\\
%$^{2}$Department, Institution, Street Address, City Postal Code, Country\\
%$^{3}$Another Department, Different Institution, Street Address, City Postal Code, Country
%}


%\and Dipartimento di Fisica e Scienze della Terra, Universita degli Studi di Ferrara, Via Saragat 1, I-44122 Ferrara, Italy 
%\and Faculty of Science and Engineering, University of Groningen,  Nijenborgh 4, 9747 AG Groningen, The Netherlands
%\and Centre for Cosmology, Particle Physics and Phenomenology, Institute of Mathematics and Physics, Louvain University, 2 Chemin du Cyclotron, 1348 Louvain-la-Neuve, Belgium
%\and Institut d'Astrophysique de Paris, GReCO, UMR7095 CNRS, 98 bis boulevard Arago, 75014 Paris, France
%\and Laboratoire d'Annecy de Physique des Particules (LAPP), Universit\'e Savoie Mont Blanc, CNRS/IN2P3, F-74941 Annecy, France
%\and Universidade de Bras\'ilia, Instituto de F\'isica, Caixa Postal 04455, Brasília, DF, 70919-970, Brazil}

%% End authors and affiliations in AA style

%PO Box 72
%9700 AB Groningen}
%\date{Received --, --; accepted -- --}


%% Authors and affiliations
%\author[ Bom et al.]{C.~R.~Bom$^{1,2}$ %\thanks{e-mail address: debom@cbpf.br}
%, J.~Poh$^{3}$
%, B.~Nord$^{3,4,5}$
%, M.~Blanco-Valentin$^{2}$
%, L. O. Dias$^{2}$
%\and Order TBD
%\\
%$^{1}$Centro Federal de Educa\c{c}\~ao Tecnol\'ogica Celso Suckow da Fonseca, Rodovia M\'ario Covas, lote J2, quadra J, CEP 23810-000,  Itagua\'i, RJ, Brazil %Distrito Industrial de Itagua\'{\i} , 
%Itagua, RJ, Brazil
%\\
%$^{2}$ Centro Brasileiro de Pesquisas F\'isicas, Rua Dr. Xavier Sigaud 150, CEP 22290-180, Rio de Janeiro, RJ, Brazil
%\\
%$^{3}$ Fermi National Accelerator Laboratory, P.O. Box 500, Batavia, IL 60510, USA
%\\
%$^{4}$ Department of Astronomy and Astropysics, University of Chicago, 5640 S. Ellis Ave., Chicago, IL 60134, USA
%\\
%$^{5}$ Kavli Institute for Cosmological Physics, University of Chicago, 5640 S. Ellis Ave., Chicago, IL 60637, USA
%}


% ====================================================================
% Introduction
% ====================================================================
%\section{Introduction Outline}
%\label{sec:introductionoutline}


% what is strong lensing?
%SL is the process by which space-time is warped, resulting in the deflection of photons as they stream from a distant source to an observer. 
%The resulting observed image is thus itself warped. 
%This requires an alignment between the distant source emitting the photons, the lens that causes the deflection, and the observer.
%Strong lenses typically occur from galaxy-scale to galaxy cluster-scale. 
%Strong gravitational lensing is the process by which a massive object distorts space-time, such that the path of a nearby photon will be deflected. 
%When observed, this results in the distortion of the image of the source object that emitted the photon. 
%The degree of warping depends on two primary factors --- the mass distribution of the deflector and the distances between the source, the deflector, and the observer; and these cosmic distances depend on the matter and energy content of the universe --- i.e., the cosmic dark matter and dark energy densities. \\
 
% why is strong lensing powerful. 
%Strong lenses are dependent on the parameters mentioned above, so they can also be probes of these parameters. 
%Galaxy-galaxy lenses; galaxy-quasar lenses with time-delays; probing dark matter haloes by stacking galaxy-galaxy lens models; the idea from Birrer about lots of einstein rings? \\

% how surveys will make lensing science newly powerful; 
%\noindent Lenses will be numerous and at different populations in upcoming surveys; DES, LSST, WFIRST, EUCLID \\
 
% lens finding models
%\noindent Discuss the multitude of new algorithms based on deep learning.\\
 
% methods for modeling 
%\noindent Modeling methods include parameterized and non-parameterized.\\
%\noindent New methods involve deep learning. %\citep{2017Natur.548..555H}\\

% challenges in modeling
%The Strong Lensing effect is sensitive to the mass distribution in the lens and the angular diameter distances involved. It is worth mentioning that this effect does not depend on the dynamical state of the object acting as lens and is also achromatic. \\

%\noindent need to model faster - enter deep nn's 

% organization of paper


% ORGANIZATION
%The paper is organized as follows. 
%In \S\ref{sec:data}, we present the simulated and real-sky data sets used in this work.
%We then describe the application of deep neural networks, including multiple architectures \S\ref{sec:measurement}. 
%In \S\ref{sec:results}, we present results of analysis on simulated data and data from DES. 
%We conclude and present an outlook for future work in \S\ref{sec:conclusion}.


%To analyze the present and future candidates would be a proibithory ammount of dedicated surveys to with might be a caveat to many scientific applications


%Quantifying image distortions caused by strong gravitational lensing and estimating the corresponding matter distribution in lensing galaxies has been primarily performed by maximum likelihood modeling of observations. This is typically a time and resource-consuming
%procedure, requiring sophisticated lensing codes, several data preparation steps, and finding the maximum likelihood model parameters in a computationally expensive process with
%downhill optimizers1


%. Accurate analysis of a single lens can take up to a few weeks and requires the attention of dedicated experts.




%Among the many Strong Lensing observables being used to constrain Cosmology we focus our attention on galaxy scale Strong Lensing. This involves% a detailed modeling of the galaxy cluster mass distribution, whose free parameters are fitted together with the cosmological parameters. %and needs to use the so-called lens inversion techniques. 
%This approach has also been explored as a powerful probe of the mass distribution in the inner cluster regions \citep[e.g.,][]{2008A&A...481...65H, 2015ApJ...800...38G}. %The many applications of inverse modelling have motivated the developments of several algorithms to derive the lens mass distribution either in a parametric way or in \textit{free-form} \citep[e.g., ][]{2009ApJ...706.1201B,2005MNRAS.360..477D, 2008ApJ...681..814C, 2010ascl.soft10012O,2007NJPh....9..447J}.
%The great number of free parameters and diverse response due different techniques, models or observational conditions led to a concern in the robustness of this type of analysis. Some authors have investigated the systematic errors arising from the models and make comparisons between the lens inversion techniques \citep[e.g.][]{2016arXiv160507621P,2016arXiv160604548M}.


%More recently, machine learning techniques that have
%become widely used in the fields of computer image processing and artificial intelligence have been applied to this
%problem and others in astronomy. In particular, artificial
%neural networks (ANNs), support vector machines (SVM),
%and logistic regression. SVMs and logistic regression methods belong to the family of reproducing kernel Hilbert Space
%methods. They learn from a training set how to classify objects using features given by predefined kernel functions.
%ANNs (and a popular variant convolutional neural networks (CNNs) ) are even more flexible in learn directly
%from a training set which features are the most important for distinguishing categories of objects. These have
%been used widely for such tasks as handwriting and facial
%recognition. In astronomy, these families of algorithms are
%beginning to be used for categorizing galaxy morphologies
%(Dieleman et al. 2015), photometric redshifts (Cavuoti et al.
%2017; Sadeh et al. 2016; Samui & Samui Pal 2017), supernova classification (Lochner et al. 2016) and the lens finding
%problem (Jacobs et al. 2017; Petrillo et al. 2017; Ostrovski
%et al. 2017; Bom et al. 2017; Hartley et al. 2017).

%These numbers will increase by one order of magnitude with the close completion of the KIDS\footnote{\texttt{http://kids.strw.leidenuniv.nl/}} \citep[KiDS;][]{KiDSr2} and DES\footnote{\texttt{http://www.darkenergysurvey.org}} \citep[DES;][]{DESnonDE}, which will cover, respectively, 1000 and 5000 square degrees with sub-arcsecond seeing. 
%Comparable numbers are expected from the ongoing Hyper Suprime-Cam\footnote{\texttt{http://www.naoj.org/Projects/HSC/surveyplan.html}} (HSC) and the forthcoming Javalambre Physics of the Accelerating Universe Astrophysical Survey \citep[J-PAS;][]{JPASredBook} projects.
%These numbers are expected to increase even further in the near future, with the operation of the Large Synoptic Survey Telescope \citep[LSST;][]{LSST20} and 
%Euclid\footnote{\texttt{http://www.euclid-ec.org/}} % http://sci.esa.int/euclid/}
%\citep{EuclidSciBook}, %WFIRST
%which are both expected to detect $\mathcal{O}\left(10^5\right)$ systems with arcs \citep{Collet2015}.
%depth: LSS, seeing/resolution: Euclid

% were obtained either by the direct visual inspection of the images of the projects mentioned above or by looking at cutouts 


%depends on the gravitational potential of the matter distribution that acts as lens and 


%Gravitational arcs have also been used to constrain the background cosmological model %, %, including Dark Energy
%both using arc statistics, modelling individual systems with large numbers of families of multiple images, or in combination with other observables
% allowing the measurement of mass profile of early type galaxyes near and at cosmological distance \citep{0004-637X-575-1-87,2002MNRAS.337L...6T,2006ApJ...649..599K}. 
%The many applications of Strong Lensing have aroused
 %{\it Strong Lensing Survey in the 
 %2005ApJ...627...32S
 %SOAR Gravitational Arc Survey \citep[SOGRAS,][]{2013MNRAS.432...73F}
%\citep[SOGRAS]{2013MNRAS.432...73F}
%the {\it Optimal Line-of-Sight-Lens Survey} \citep[OLS;][]{2006MNRAS.369.1521W},


%This is true for the targeted surveys and also for the wide-field imaging surveys, where either the full footprint or cutouts 
%around potential lenses (e.g., luminous red-galaxies, galaxy clusters) are visually inspected. In section \ref{visual_inspection} we discuss the visual inspection approach in which we participated using Dark Energy Survey Science Verification data \citep{DESSL1Nord}, which covered an area of $250$-sq-deg. 

%-- Strong Lensing Legacy Survey} 



%In order to do so, and as \cite{gal2016dropout} suggest, we apply a random binomial noise (binary mask) to every weight layer (in this case, convolutional and dense layers), for every sample, thus forcing the net to learn how to extract features from the input data redundantly while training, so that if random weights of the layer itself are dropped (and so they do not contribute to that layer's response) the resulting activation map still minimizes the regression error.

%By employing this approach, even identical samples can generate prediction outputs which may vary within a certain interval (the smallest the interval, the lower the model error and thus the higher its predictive confidence for that specific sample). If a sufficient number of predictions are obtained for any given input sample, it is possible then to obtain an approximation of the probability distribution function of that specific predicted property for that sample. Figure \ref{fig:bayesianerror} shows an example of how this methodology works: The same input data (lens image) is introduced $k$ times into the same deep model; each time the data is introduced into the model different random binomial noise masks are applied to the weight layers of the model; applying these masks causes each output to be different (the amount of variation of the output depends on how the model was trained); the $k$ estimated values can be used to obtain an approximation of its probability distribution function (frequency of estimations).


%\figurebayesianerrorexplanation



% --------------------------------------------------------------------
% SubSection: Dark Energy Survey Data
% --------------------------------------------------------------------
%\subsection{Dark Energy Survey}
%\label{sec:darkenergysurvey}

% The below has to be re-worded, because this is copied from another paper I wrote.
%DES is a deep sky survey covering $\sim5000$ \sqdeg\ of the southern Galactic Cap in five optical filters ($grizY$). 
%It includes a wide-field survey to a depth of $i\sim24$ mag at $10\sigma$ detection threshold, as well as a 30\sqdegadjective\ supernova survey spread over 10 fields --- eight shallow and two deep. 
%The depth in the repeated supernova area is typically two magnitudes deeper than the wide-field survey. 
%DES uses the Dark Energy Camera \citep[DECam][]{flaugher15}, a wide-field (or 3-sq.-deg.) CCD mosaic camera located on the Blanco 4m telescope at the Cerro Tololo Inter-American Observatory in the Chilean Andes. 
%The DES footprint is visible between August and mid-February. 
%Each year, DES is allocated $\sim105$ nights, and it has now completed five years of planned observations. 
%DECam is particularly suited to high-redshift survey work due to its large field of view and red-sensitive CCDs.

%For this work, we use the Year One First Annual (Y1A1) internal collaboration release of the DES data. 
%The survey and operations are described in \citet{diehl14}. 
%The data contained in the Y1A1 release were taken between 2013 August 15th and 2014 February 9th. 
%These data cover $\sim1840$ \sqdeg\ to a median $10\sigma$ point source (MAG PSF) depth in AB magnitudes of 23.28, 23.6, 23.1, 22.3 and 20.8 in the $g$, $r$, $i$, $z$, and $Y$ bands, respectively. 

%The DES data management (DESDM) team was responsible for the reduction of Y1 images.  
%The detrended, single-epoch images were calibrated, background-subtracted, and combined into `coadd tiles.'
%The tiles are coadd images comprising one to five exposures in each of the five wavebands, with an average coverage of 3.5 exposures for each tile. 
%Each coadd tile has dimensions $0.73\ {\rm deg.}\times 0.73\ {\rm deg.}$, so defined as to cover the entire DES footprint homogeneously. 
%The Y1A1 release is shallower than the final survey depth and consists of 3707 coadded tiles covering two non-contiguous regions---one overlapping the deeply imaged Stripe 82 \citep{jiang14} from SDSS \citep{york00, abazajian09}, and one overlapping with the area covered by the South Pole Telescope \citep[SPT;][]{carlstrom11}. 
%More details of the reductions are available in \citet{drlicawagner17arxiv}. %ADW paper also discusses star-gal classification

%Catalog source detection uses the Source Extractor \citep[][]{bertin96, bertin11} image detection software in double-image mode using the $\chi^2$ detection image constructed from the combination of the $r$, $i$, and $z$ band images, as the detection image. 
%Unless otherwise stated, photometric and position data of all objects in this work (see Table~\ref{table:lensingobjects}) originate in this object catalog. We use the magnitude measure, \nord{\texttt{Mag\_Auto}, which suffers from segmentation issues and so the magnitudes cannot be used for stellar mass.}

%DES DR1 is ... 
% https://des.ncsa.illinois.edu/releases/dr1
%https://arxiv.org/abs/1801.03181
%https://des.ncsa.illinois.edu/releases/dr1/dr1-docs

%\subsubsection{Lens Samples}

%We use a sample lenses that exist in the DES footprint, and that have been confirmed and measured. We use DES images to perform the CNN regression measurement, and then compare to the independent measurements from the literature. Please see TableXX for a list of these systems and their parameters of interest. 


% --------------------------------------------------------------------
% SubSection: Training
% --------------------------------------------------------------------

%\subsection{Data Set Preparation}
%We used two different sources of data to train and test our model. The first dataset consists on $18,600$ samples of simulated lens systems, with different parameters and configurations. The I, R and G channels for the original image, as well as the image with the source galaxy subtracted, are available for each sample.

%Apart from that, the information regarding 22 different lensing properties were available for each datasample (among of which the estimated properties presented on this paper were also available: lens redshift, source redshift, einstein radius, lens velocity and distance ratio).

%The second dataset consists on $17$ samples of real lens systems. The same channels as in the first dataset are available for this one, however no source galaxy subtracted images were available when writting this work. All these $17$ samples were used to test the network only (they were not used while training the net). 
%\subsubsection{how long does it take to do inference}
%Table \ref{tab:inferencetime} shows the total time required to obtain the inference results for all testing samples, using a total number of inferring runs of $1,000$ per sample.
%\subsubsection{what machine was this run on, and how long did it take?}

%Table \ref{tab:numepochs} shows the number of epochs each architecture took to be trained for each parameter estimated, using the configuration specified previously, while Table \ref{tab:trainingtime} shows the total training time for each case.

%Two parameters are used for making the Bayesian inference possible on each dropout layer: the weight and the dropout regularizers. Both of them were set to the values proposed by \cite{gal2016dropout}. 


% ................
% put tables here.

% ......
% add figure of loss history




% ====================================================================
% Section: Results
% ====================================================================


%fig:sam_in
%fig:zs_in
%fig:zl_in
%fig:vd_in
%fig:er_in



% ====================================================================
% Section: Conclusion
% ====================================================================


% ====================================================================
% Section: Conclusion
% ====================================================================

%The uncertainty in real dataset may also suffer some caveats and not be as low as in the current results since this simulations are idealized........  When dealing with real images one would also have take into account uncertainties that might appear due to this idealization, i.e.,  effects due the \textit{heterostatic} data. In such regime one need to proper estimate the \textit{aleatoric} uncertainties from the data instead of simply fine tuning it. One possibility to reduce the uncertainties effect of \textit{heterostatic} data might be if one could do \textit{transfer learning}, i.e. start from the models presented in this paper and make a fine tuning, or retraining in real data. Since there are orders of magnitude fewer examples in real data, to properly train this scheme one might also need to make use data augmentation methods. This is currently under investigation and will be addressed in a following paper.



%* we also tested a resnet, however, as the resnet acts as an emsamble of sequential nets ists results are very stable even using the concrete dropout method, the errorbars derived were unrealistic smaller if compared to the actual deviation from truth values and suggesting a bias.

%* The algorithm is modeling SL ?

%General conclusions and future work: 
%We could really train a supervised deep learning framework and derive estimations of velocity dispersion, lens redshift, einstein radius using 3 bands ONLY with sims considering a realistic population of Strong lensing. In some regions, we achieved a estimation below $10\%$ error.
%However even if we remove the Lens images, the source redshift is poorly estimated.

%This is important because: We will not have high quality imaging and spectra for all strong lensing in the current surveys and forthcoming.

%There is a bias in the regions we have small number of lenses
%To give reliable results in real data one must make a fine tuning using real data in order to overcome the idealization of our sims. Couple of ideias: Transfer Learning, GANN agumentation to deal with the small ammount of real lenses, more sims in the regions we have small number os lenses. Tuning with semi-supervised learning using some 
%Increase the sample of real data available





